"I Don't Think So": Summarizing Policy Disagreements for Agent Comparison

With Artificial Intelligence on the rise, human interaction with autonomous agents becomes more frequent. Effective human-agent collaboration requires users to understand the agent's behavior, as failing to do so may cause reduced productivity, misuse or frustration. Agent strategy summarization methods are used to describe the strategy of an agent to its destined user through demonstration. A summary's objective is to maximize the user's understanding of the agent's aptitude by showcasing its behaviour in a selected set of world states. While shown to be useful, we show that current methods are limited when tasked with comparing between agents, as each summary is independently generated for a specific agent. In this paper, we propose a novel method for generating dependent and contrastive summaries that emphasize the differences between agent policies by identifying states in which the agents disagree on the best course of action. We conduct user studies to assess the usefulness of disagreement-based summaries for identifying superior agents and conveying agent differences. Results show disagreement-based summaries lead to improved user performance compared to summaries generated using HIGHLIGHTS, a strategy summarization algorithm which generates summaries for each agent independently.

==> Rebuttal.tex <==

\clearpage

\section{General Response}
We thank the reviewers for their feedback. We first address concerns that appeared in multiple reviews, then reply to each reviewer's specific comments separately.
\\
\textbf{Choice of HIGHLIGHTS as a baseline}
Prior work has shown that HIGHLIGHTS outperformed several baselines (Amir \& Amir 2019, Huber et al. 2021). Another approach for generating summaries is through machine teaching (Lage et al., 2019, Huang et al., 2019), but it requires making assumptions about  users’ generalization, and does not scale computationally so could not be applied to these domains. Other summary criteria were proposed by Sequeria \& Gervasio (2020) but they were not evaluated in the context of comparing agents and there was also no clear approach that outperformed others. As such, and since the main goal of the paper was to demonstrate the potential benefit of moving from independent summaries to summaries that contrast two agents, HIGHLIGHTS was the most prominent baseline.

\textbf{Simulator requirement}
% While our approach assumes access to a simulator, this does not have to be the case.
% Following the Leader’s execution plan while simultaneously querying the Disageer to identify disagreements is applicable in real-world scenarios by determining importance based solely on the disagreement state. Using trajectory-based disagreements could prove to be more difficult, as allowing the Disagreer to branch out and revert back to the disagreement state might not be feasible in some real-world domains.
We agree that the need for a simulator limits the ability to use the approach on any provided agent. However, as long as there's a way to query the agent for its actions given a state, the agents do not have to be trained using the same simulator. This is a first step toward enabling agent comparison, a problem which has not been directly addressed by prior work. The current approach could support developers and allow them to share summaries with domain experts that collaborate with them and end users who wish to compare different policies. We note that all existing approaches require a simulator, and compared to these, we require fewer assumptions (e.g., an additional causal model (Miller 2020) or access to the agent's training as required for reward decomposition and saliency maps). 


\paragraph{Response to R1:}
\textbf{Contribution and advantage over multiple HIGHLIGHTS}
The underlying research question is supporting comparison of alternative agents. The proposed solution provides a conceptual contribution rather than an increment to  HIGHLIGHTS,  motivated by literature in cognitive science which suggests that contrastive explanations are typically more helpful to people than only showing a chosen action. We followed this approach to compare two policies.
% The comparisons generated by our approach are contrastive, compare the agents in equivalent scenarios, algorithmically locate and display only divergence in agent policies and do not require the user to watch numerous different test cases which might be  time-consuming and tedious.
The user study demonstrates the benefit over using separate HIGHLIGHTS summaries as DISAGREEMENTS summaries led to higher correctness rates in users' evaluations of agents.
Computational efficiency-wise, the  approaches are similar, as both require running simulations of the agent and ranking of states. 

\textbf{Motivation example}
Safety over speed is an example for cases where agents may prioritize different outcomes.


\textbf{Claim that other approaches are not optimized for the task}
We were referring to other global explanations, claiming they are not tailored to support a particular user need, e.g., debugging an agent, collaboration, or the need we address here - comparing alternative policies.

\paragraph{Response to R2:}
\textbf{Supported MDPs}
Any MDP can be used. In particular, the highway domain has a continuous state space. Currently, the approach only supports discrete actions, but it could be extended to a continuous action space by clustering actions, or defining distances between actions.


\paragraph{Response to R3:}
\textbf{Works on reconciling a user's expected policy}
We are not sure which works the reviewer refers to, we would be happy to add discussion of any additional related works we've missed. 

\textbf{Success rate using HIGHLIGHTS}
We explain this in the results section: \textit{``We hypothesize that these responses are a consequence of a single trajectory in agent E’s summary [...] These results emphasize the limitations of independent comparisons.''}

\textbf{Rescaling Q-values}
While the q-values may differ due to the rescaling, the selected action of each agent is unaffected, therefore the disagreements themselves are still viable.
We agree that the scaling might need to be fitted for particular domains. In the domains we used we conducted sensitivity analyses to make sure their effect is not substantial.

\textbf{Last state importance}
The chosen criteria for disagreement importance identifies trajectories where the agents (while possibly prioritizing alternative outcomes) agree that one of them has reached a poor state while the other a desirable one. The reason it was chosen was to provides a shared ground truth regarding the states the agents arrive at.
We considered other importance functions which were left out due to space limitations, we will add those to the Appendix.

\textbf{Proxy metrics vs. human studies}
Our goal is to support users and it is unclear what computational metric could serve as a proxy for this outcome. We did conduct sensitivity analyses computationally to test the affects of parameters on the output summaries. 


\paragraph{Response to R4:}
\textbf{soundness of user studies.}
To be as confident as possible in our findings, we followed key principles of experimental design (e.g., choice of evaluation metrics that answer the research question, random assignment to conditions, testing of participants’ attention and understanding of the task, use of multiple domains, comparison to a meaningful baseline). 

\textbf{Addressing continuous or vast state space}
We overcame this challenge by observing all disagreements in a sampled set of trajectories. The number of samples is configurable.

\textbf{Filtered participants}
The reported number of participants is after filtering. We excluded 3 participants.

\textbf{Participant proficiency}
No significant differences were uncovered by these questions, we will add this to the Appendix.

\textbf{No statistical differences in confidence and satisfaction}
Our null findings with respect to confidence and satisfaction are in line with some other prior studies that showed that even when significant performance differences were found, this was not always reflected in participants’ confidence in their answers (Amir \& Amir 2019). Since these are subjective measures, it is also possible that the between-subject design reduces our ability to observe such differences (if variance between participants in these aspects is greater than the effect of the intervention).

\textbf{Requirement of access to the policy}
It is true we need such access. One idea to overcome this would be to use Inverse RL methods to retrieve an estimate of an agent's policy and then apply our approach to it. 




==> sections/abstract.tex <==
\begin{abstract}
With Artificial Intelligence on the rise, human interaction with autonomous agents becomes more
frequent. Effective human-agent collaboration requires users to understand the agent's
behavior, as failing to do so may cause reduced productivity, misuse or frustration. Agent strategy summarization methods are used to describe the strategy of an agent to its destined user through demonstration. A summary's objective is to maximize the user's understanding
of the agent's aptitude by showcasing its behaviour in a selected set of world states. While shown to be useful, we show that current methods are limited when tasked with comparing between agents, as each summary is independently generated for a specific agent. In this paper, we propose a novel method for generating dependent and contrastive summaries that emphasize the differences between agent policies by identifying states in which the agents disagree on the best course of action. 
% We conduct user studies to assess both the affect of our method on an agent selection task and on an agent understanding task.
We conduct user studies to assess the usefulness of disagreement-based summaries for identifying superior agents and conveying agent differences. 
Results show disagreement-based summaries lead to improved user performance compared
to summaries generated using HIGHLIGHTS, a strategy summarization algorithm which generates summaries for each agent independently.
\end{abstract}

==> sections/approach_methods.tex <==
\section{Disagreement-Based Summaries}
We propose a new summary method which supports the comparison of alternative
agents by explicitly highlighting the \emph{disagreements} between them. Thus,
constructing \emph{contrastive} summaries that convey policy divergence between
agents exposed to the same world states. This approach is in line with the
literature on explanations from the social sciences, which shows that people
prefer contrastive explanations \cite{miller2018explanation}. We note that while
typically contrastive explanations refer to ``why not?'' questions and consider
counterfactuals, in our case the contrast is between the decisions made by two
different policies.

We next describe our proposed disagreement-based summary method. Specifically,
we formalize the notion of agent disagreement,
describe the ``\disalg~'' algorithm for generating a joint summary of the
behavior of two agents, and describe how to measure the importance of a disagreement state and disagreement trajectory.


\paragraph{Agent Disagreement}
%%%%%%% define a disagreement %%%%%%%
The two main dimensions on which agents can differ are their valuations of
states and their policies, i.e. their choice of action. These dimensions are of
course related, as different state valuations will naturally lead to different
policies. Our definition of a disagreement focuses on the policy. We then utilize the value function for ranking purposes.

In other words, any state $s$ for which different agents choose different
actions is considered a disagreement state. We use these states to
analyze and portray how the agents differ from one another in their behavior.
Formally:
\begin{definition}[Disagreement State]
    Given two agents ${Ag}_{1}$ and ${Ag}_{2}$ with policies  $\pi_1, \pi_2$,
    respectively. Define a state $s$ as a disagreement state $s_D$ iff:
    \begin{align}
        \pi_1(s) \neq \pi_2(s)
    \end{align}
    The set of all disagreement states $\mathbb{D}$ would then be:
    \begin{align}
        \forall s \in S \; | \; \pi_1(s) \neq \pi_2(s) : s \in \mathbb{D}
    \end{align}

\end{definition} 


%%%%%%% continuous or vast domains %%%%%%%
For a compact MDP where every state may be computed, this definition would
suffice. Alas, for more complex settings containing a continuous or vast state
space, it is not feasible to compare all states. The proposed method must be
able to overcome this difficulty.

%%%%%%% How to compare agents? %%%%%%%
\paragraph{Identifying Agent Disagreements Through Parallel Online Execution}
Given two alternative agents to compare, we initiate an online execution of both
agents simultaneously such that we follow the first (denoted as the
\emph{Leader} or $L$ for short, with policy $\pi_{L}$), while querying the
second (denoted as the \emph{Disagreer} or $D$ for short, with policy $\pi_{D}$)
for the action \emph{it} would have chosen in each state. Both agents are
constrained to act greedily and deterministically with respect to their
$Q$-values. Upon reaching a disagreement state, we allow the \emph{Disagreer} to
``split-off'' from following the \emph{Leader} and continue independently for a
limited number of steps while recording the states it reaches for later
analysis. Once the limit is reached, we store the \emph{disagreement
trajectory}, and revert the \emph{Disagreer} back to the disagreement state,
from which it continues to follow the \emph{Leader} until the next disagreement
state is reached and the process is repeated.

\paragraph{The \disalg~ Algorithm}
The algorithm pseudo-code is supplied in Algorithm \ref{alg:disagreements}. It's parameters are summarized in Table \ref{tb:parameters}. 

\begin{table}[ht]
    \centering
    \small
    \resizebox{0.85\columnwidth}{!}{%
    \begin{tabular}{|p{1.6cm}|p{4cm}|p{0.5cm}|p{0.5cm}|}
    \hline
    \textbf{Parameter} & \textbf{Description} & \textbf{F} & \textbf{H}
    \\
    \hline
    $k$ & Summary budget, i.e. number of trajectories & 5 & 5 \\
    \hline
    $l$ & Length of each trajectory & 10 & 20 \\
    \hline
    $h$  & Number of states following $s$ to include in the trajectory &5& 10  \\
    \hline
    $numSim$ & The number of simulations (episodes) run by the \disalg~ algorithm &10&10  \\
    \hline
    $overlapLim$ & Maximal number of shared states allowed between two trajectories in the summary & 3& 5 \\
    \hline
    $impMeth$  & Importance method used for evaluating disagreements & \emph{Last State} & \emph{Last State}\\
    \hline
    \end{tabular}}
    \caption{Parameters  for Frogger \& Highway domains.}
    \label{tb:parameters}
\end{table}

%%% explaining the algorithm
\emph{The Algorithm.} First, three lists are initialized for the Leader traces,
disagreement states and Disagreer trajectories (lines 4--6). Then, simulation of the agents are run (lines 7--27). Each simulation collects all
states seen by the Leader during the execution (line 24), disagreement states
(line 13), and the Disagreer trajectories (lines 14--19). Each step of the
simulation, both agents are queried for their choice of action (lines
10--11), if they disagree on the action --- a disagreement state is added
(line 13) and a disagreement trajectory is created (lines 14--19), after which
the simulation is reverted to the last disagreement state (line 21). Upon simulations completion, all disagreement trajectories (coupled pairs of
Leader and Disagreer trajectories) are obtained (line 28) and the most important ones are passed as output (line 29).   



\begin{algorithm}[tb]
    \caption{The \disalg~ algorithm. }
    \label{alg:disagreements}
\begin{algorithmic}[1]
    %\vspace{-0.2cm} \SetAlFnt{\small\sf} \DontPrintSemicolon % Some LaTeX
    % compilers require you to use \dontprintsemicolon instead
    \STATE {\bfseries Input:} $\pi_L,\pi_D, k, l, h,$ \STATE $overlapLim,
    numSim, impMeth$ \STATE {\bfseries Output:} $\mathbb{S}$ \STATE $L_{Tr}
    \leftarrow$ empty list \textit{\;\;\;\#Leader traces} \STATE $\mathbb{D}
    \leftarrow$ empty list \textit{\;\;\;\#Disagreement states} \STATE $D_T
    \leftarrow$ empty list \textit{\;\;\;\#Disagreer trajectories}  \FOR
    {$i=1$ {\bfseries to} $numSim$} \STATE $sim, s = InitializeSimulation()$
    \WHILE {$(!sim^{\pi_L}.ended())$} \STATE $a^{\pi_L} \leftarrow
    sim.getAction(\pi_L(s))$ \STATE $a^{\pi_D} \leftarrow
    sim.getAction(\pi_D(s))$ \IF{$a^{\pi_L} != a^{\pi_D}$} \STATE
    $\mathbb{D}.add(s)$ \STATE $d_t \leftarrow$ empty list
    \textit{\;\;\;\#Disagreer trajectory} \FOR{$i=1$ {\bfseries to} $h$}
    \STATE $s^{\pi_D} \leftarrow sim.advanceState(\pi_D)$ \STATE $a^{\pi_D}
    \leftarrow sim.getAction(\pi_D(s))$ \STATE $d_t.add(s)$ \ENDFOR \STATE
    $D_T.add(d_t)$ \STATE $sim, s = reloadSimulation(D_s[-1])$ \ENDIF \STATE $s
    \leftarrow sim.advanceState(\pi_L)$ \STATE $L_{traces}.add(s)$ \ENDWHILE
    \STATE $runs = runs+1$ \ENDFOR \STATE $DA_T \leftarrow
    disagreementTrajPairs(\mathbb{D},L_{Tr}, D_T, l, h)$ \STATE $\mathbb{S}
    \leftarrow topImpTraj(DA_T, k, overlapLim, impMeth)$
    \end{algorithmic}
\end{algorithm}


Since the \emph{Leader} agent controls which areas of the domain state-space are reached, we repeat the process again, reversing the agent's roles. This is important because the Leader determines which regions of the state-space are reached and as such also conveys information about the agent's preferences. This process results in two sets of disagreements states (one for each agent as the \emph{Leader}). Typically, these sets can be very large, and it is infeasible for a user to explore all of them. 
% Upon termination, an output summary is required. To exempt our user from examining all (potentially numerous) disagreements, we limit the summary to display a fixed number of disagreement states. 
Therefore, a ranking procedure is
necessary for the disagreements found in order to generate a compact summary. We next describe approaches for
quantifying the importance of a disagreement.


% \subsection{The ``\disalg~'' Algorithm}
% The algorithm initializes a Leader and Disagreer agent to run simultaneously in
% an identical environment.The Leader decides which action is best to initiate and
% both agents execute it, such that their progression and relative environments
% remain identical. At each time-step, the Disagreer proposes the action it would
% have taken given the choice. A state where the agents disagree on the best
% action is defined as a disagreement state. Upon reaching a disagreement, the
% disagreer branches off to progress on its own for a limited number of time-steps
% while recording the trajectory, after which it reverts back to the disagreement
% state and continues to follow the Leader. Upon termination of the Leader's
% execution, all disagreement states and branching trajectories are ranked and
% used to generate a summary.


%%%% Disagreements algorithm pseudo code


\paragraph{Disagreement Importance} 
Various methods can be used for determining disagreement importance. We first define the notion of a state's value based on multiple
agents.

\textbf{State Value}
% Each agent possesses an internal valuation function, assigning values to states
% or state-action pairs.
We assume the agents are $Q$-based, possessing a $Q$ function ($Q(s,a)
\rightarrow \mathbb{R}$) which quantifies
their valuation of state-action pairs, denoted as $Q$-values. $Q$-values are calculated and adjusted during the
training phase of the agent and depend on the algorithm used as well as on the
specification of the reward function. Therefore, $Q$-values of different agents
may vary greatly. This renders each individual agent's assessment of a
state-action pair as its own estimate rather than representing a ground truth.
The values themselves may not even be on the same scale. To allow for comparison
between values, we normalize each agent's $Q$-values by dividing by the maximum
$Q$-value appearing in each, thus rendering each value an indication of how good
a state-action pair is compared to the best one observed by the agent. Formally:
\begin{align}
    Q' = \frac{Q-\min_{s,a} \big(Q(s,a) \big)}
    {\max_{s,a} \big (Q(s,a) \big )- \min_{s,a} \big(Q(s,a) \big)}  
\end{align}

Since our agents' action selection is greedy and deterministic with respect to
their $Q$-values, we denote the value of state $s$ as the highest
$Q$-value associated with it.
 \begin{definition}[Agent State Value]
    Given an agent $Ag$, its $Q$ function $Q^{Ag}$ and a state $s$, we define
    the value of $s$ as:
    \begin{align}
       V^{Ag}(s) = \max_a {Q'}^{Ag}(s,a)
    \end{align}
 \end{definition} 


% % We now discuss the different methods available for measuring disagreement
% % importance.
% \paragraph{Disagreement Extent}
% Any state where the next action of the compared agents differs is a disagreement
% state, but not all disagreements are of the same magnitude. For instance,
% consider a scenario where both agents wish to arrive at a location that is
% diagonally above them and to the right. One agent chooses to first go \emph{up}
% while the other chooses to go \emph{right}. It is reasonable then to assume that
% each agent's assessment for the other's action was not far from that of the
% action it chose to take. We would like to define disagreement extent as a metric
% for predicting the impact of a specific disagreement. We define the notion of an
% agent's confidence in an action $c^{{Ag}}(s,a)$ as the probability that this
% action is the optimal one to take in the current state, proportional to all
% other action possibilities. Formally:
% \begin{align}
%     C^{{Ag}}(s,a) = \frac{Q'^{{Ag}}(s,a)}{\sum_{i=1}^{|A|} Q'^{{Ag}}(s,a_i)} 
% \end{align}

% Using this notion, we propose a measure for disagreement extent based on the
% confidence of each agent in their choice of action compared to the action
% selected by the other agent.  

% \textbf{BeTY - Better Than You}: Given the Leader and Disagreer agents $L$,
% $D$, a disagreement state $s \in \mathbb{D}$, and the actions chosen by each of
% the agents denoted $a_{L} = \pi_{L}(s)$ and $a_{D} = \pi_{D}(s)$, we propose
% measuring the significance of the disagreement by querying each agent not solely
% about its confidence in its choice but, in addition, how confident it is that
% the rival's choice of action is poor. 

% The BeTY importance is then Formally: 
% \begin{align}
%     Im(s)_{BeTY} = |C^{L}(s,a_{L}) -  C^{L}(s,a_{D})| \nonumber  \\
% + |C^{D}(s,a_{D}) - C^{D}(s,a_{L})|
% \end{align}

% Now we are able to quantify the extent of the disagreement as dependent on both
% agents' evaluations.

% Alas, measuring only the importance of the disagreement state has its
% limitations. Without ground truth regarding the quality of the disagreeing
% actions we are left only with the agents' estimations which may be flawed.
% Suppose our agents reach a disagreement state where the disagreement extent is
% high, i.e. in the case of \emph{BeTY}, where both agents think the other is
% making a lousy choice. They each go their separate ways but reunite at a shared
% state after taking several actions with minimal to no impact on the succeeding
% execution. This realization led us to formulate another approach for determining
% the importance of a disagreement state. 

Alas, measuring only the importance of a single state has its limitations.
Without ground truth, we are left only with the agents' estimations which may be
flawed. Suppose our agents reach a disagreement state where both are convinced
the other's action is a poor choice. They each go their separate ways only to
reunite at a shared state after several steps with minimal to no impact on the
succeeding execution, e.g. overtaking a vehicle from the left or from the
right. This realization led us to formulate a trajectory-based approach for
determining the importance of a disagreement state. 

\paragraph{Disagreement Trajectory Importance}
To determine the importance of a disagreement state, we compare the trajectories
that branch out of it by following each agent. We formulate trajectory value
metrics to evaluate these, while constraining ourselves to observing only
trajectories of similar length.

A trajectory ${t}_{h}^{\pi}(s) = \langle s_{+1}, ..., s_{+h} \rangle$ denotes
the sequence of states encountered when following state $s$ for $h$ steps
according to a policy $\pi$. Since each agent evaluates states differently, we
consider the value of a state as the sum of both agents' valuations, i.e. $V(s)
= V^{L}(s) + V^{D}(s)$. There are numerous ways to quantify the importance of a
trajectory. A description of several methods tested in our work is provided in
the Appendix. The summaries generated for the user studies made
use of the \emph{last-state} importance method. 


\textbf{Last State Importance:}
We define the importance of a disagreement
trajectory as the difference between the values of the last states reached by
each of the agents. This reflects how ``far off'' from each other the
disagreement has led the agents. Formally:
\begin{align}
    Im({t}_{h}^{\pi_{L}}(s),{t}_{h}^{\pi_{D}}(s)) = 
    |V(s^{\pi_L}_{+h}) - V(s^{\pi_D}_{+h})|
\end{align}
This metric achieves a high importance score when one agent arrives at a state
which both agents agree is valuable, while the other agent arrives at a state whose value both agents agree is poor.


\paragraph{Trajectory Diversity}
Using these methods we are able to acquire the set of disagreement states
$\mathbb{D}$ ordered by importance, and for each, their corresponding
trajectories. These shall be woven together to create a visual summary for
displaying to the user. To increase the coverage of the summary and avoid
showing redundant trajectories (in both methods), we restrict the summary generated to not contain
\emph{i)} multiple trajectories that end or begin at the same state, \emph{ii)}
trajectories where the Leader and Disagreer share the same state before-last
and \emph{iii)} overlapping trajectories which share more than a predefined
number of states. 




==> sections/background.tex <==
\section{Related Work}
In recent years, explainable AI has regained interest, initially focusing mainly
on explaining supervised models. More recently, research has begun
exploring explanations of reinforcement learning agents~\cite{XRL_survey,
heuillet2021explainability}. 
% Some explanation methods attempt to convey the agents' reasoning when
% selecting actions, e.g. using decision-trees~\cite{liu2018toward} or causal
% models~\cite{madumal2020explainable}.
In this work, we focus on global explanations that aim to describe the policy of
the agent rather than explain a particular action. Specifically, we develop a
new method for strategy summarization. In this section we describe in
more depth strategy summary methods~\cite{amir2019summarizing}. 


% % decision trees Decision trees are popularly known for their high
% interpretability, \citet{liu2018toward} described a novel method for mimicking
% a Deep Reinforcement Learning (DRL) model by using a continuous tree
% representation (LMUTs) and interpreting it by analyzing the knowledge stored
% in the tree structure.\\
% % causal graphs Harnessing the inherent explainability of causality methods,
% \citet{madumal2020explainable} introduce and formalize an action influence
% model for model-free RL based on a structural causal model received as input
% (e.g. a DAG). The action influence model provides the ability to approximate
% the causal model of the environment relative to actions taken by the agent,
% enabling the generation of contrastive explanations for questions sch as
% ``why?'' as well as ``why not?''.\\

% In this work we develop a new method for policy summaries, therefore, in this
% section we describe in more depth policy summary methods. \oa{start with a
% more general paragraph about explainable RL (can steal from the intro and
% elaborate a bit. So it will be something like "In recent years, explainable AI
% has regained interest, initially focusing mainly on explaining supervised
% models. More recently, a line of research has begun exploring explanations of
% reinforcement learning agents. [[describe some methods]]. In this work we
% develop a new method for policy summaries, therefore, in this section we
% describe in more depth policy summary methods. Then move to your next
% paragraph}

Strategy summarization techniques convey agent behavior by demonstrating the
actions taken by the agent in a selected set of world states. The key question
in this approach is then how to recognize meaningful agent situations.

One such approach called HIGHLIGHTS~\cite{amir18highlights}, extracts
\emph{important} states from execution traces of the agent. Intuitively, a state
is considered important if the decision made in that state has a substantial
impact on the agent's utility. To illustrate, a car reaching an intended highway
exit would be an important state, as choosing a different action (continuing on
the highway) will cause a significant detour. 
% The algorithm also considers the diversity of states in the summary to avoid
% showing redundant information. 
HIGHLIGHTS has been shown to support people's ability to understand the
capabilities of agents and develop mental models of their behavior
~\cite{amir18highlights,Tobias}. 

%OFra: removed Tobi since it's not super related here. Only added him to the
%studies showing highlights results.

% %% Tobias work \citet{Tobias} combined global and local explanation methods by
% integrating HIGHLIGHTS summaries with saliency maps depicting the attention of
% the agent. They found mixed results with respect to the contributions of
% saliency maps, but reinforced earlier results regarding the effectiveness of
% HIGHLIGHTS in conveying agent behavior to people.\\

% \citet{Sequeira2020} extended HIGHLIGHTS by suggesting additional importance
% criteria for the summary state selection. These are referred to as
% \emph{Interestingness Elements} --- domain independent criteria obtained through
% statistical analysis of an agent's interaction history with the environment over
% the training sessions. Their user study did not reach clear conclusions as to
% which criteria is optimal, rather they suggest that a combination of elements
% enables the most accurate understanding of an agent’s aptitude in a task.

% Other works have proposed a different approach for generating summaries, based
% on machine teaching approaches~\cite{huang2017enabling,lage2019exploring}. These
% methods' underlying idea is to select a set of states that is optimized to allow
% the reconstruction of the agents' policy using imitation learning or inverse
% reinforcement learning methods. While such approaches are computationally
% appealing, as they rely on computational principles rather than heuristics, in
% practice they were shown to be limited. Specifically, participants' performance
% in predicting agent behavior was inferior to that of computational approaches.
% This is largely associated to the use of different state representations and
% computational models from those assumed by summary generation algorithms
% \cite{lage2019exploring}.


\citet{Sequeira2020} extended HIGHLIGHTS by suggesting additional importance
criteria for the summary state selection referred to as \emph{Interestingness
Elements}. \citet{huang2017enabling,lage2019exploring} proposed a different
approach for generating summaries based on machine teaching methods. The key idea underlying this approach is to select a set of states that is optimized to allow
the reconstruction of the agents' policy using imitation learning or inverse
reinforcement learning methods.

%Ofra: removed for space reasons, and because we do not address these
% limitations in this work Prior work \cite{amir18highlights, Tobias} showcased
% that policy summaries can help users assess agents' capabilities, but also
% revealed some limitations. People's performance in predicting agent behavior
% was lower than that of computational approaches, because they often used
% different state representations and computational models from those assumed by
% summary generation algorithms \cite{lage2019exploring}. In addition, showing
% unrepresentative demonstrations of agent behavior can lead users to make wrong
% inferences, emphasizing the need to design methods that allow people to
% proactively explore the agent's policy. \\

Common to all previous policy summarization approaches is that each summary is
generated specifically for a single agent policy, independent of other agents.
This can hinder users' ability to compare agents, as the
summaries might show regions of the state-space where the agents act similarly,
failing to capture useful information with respect to where the agent policies
diverge. For example, HIGHLIGHTS focuses on ``important'' states and it is
likely that the states found to be most the important to one agent will be
considered important by another agent as well. These could be inherently
important stages of the domain such as reaching the goal or evading a dangerous
state. If the agents act similarly in these important states, the HIGHLIGHTS
summaries of the agents might portray similar behavior, even for agents whose
global aptitude varies greatly. In contrast, if the summaries do differ from
one another and portray different regions of the state-space, they do not convey how
the alternative agent would have acted had it been tasked with the same
scenario.
% Additionally, when the summaries of different agents cover different regions
% of the state-space, they do not convey to the user what an agent would have
% done had it encountered situations shown in the other agent's summary. 

% if different behavior is attained in the summaries, it remains unclear how the
% other agent would have acted in a scenario encountered by the other agent.
% summaries of different agents demonstrate their behavior in different states,
% they still do not convey to the user what the other agent would have done had
% it encountered that particular state. 
To address these limitations, we propose a new approach that is specifically
optimized for supporting users' ability to distinguish between policies.  

% While shown to be effective in conveying agent aptitude to users, the
% HIGHLIGHTS algorithm \cite{amir18highlights} has several caveats when applied
% as a method for comparing different agents. First, HIGHLIGHTS generates an
% \emph{independent} summary of important states in a given domain for each of
% the agents. Therefore, it is likely that the states found to be of most
% importance to one agent may be considered important by another agent as well.
% These could be inherently important stages of the domain such as reaching the
% goal or bypassing a dangerous state. If the agents act similarly in these
% important state, the HIGHLIGHTS summaries of the agents could portray similar
% behavior, even for agents that have different policies in many other parts of
% the state-space. Furthermore, even if the HIGHLIGHTS summaries of different
% agents demonstrate their behavior in different states, they still do not
% convey to the user what the other agent would have done had it encountered
% that particular state. 

% These can be thought of as \emph{contrastive} summaries, as they show where
% the agents' policies diverge. This approach is in line with the literature on
% explanations from the social sciences, which shows that people prefer
% contrastive explanations \cite{miller2018explanation}. We note that while
% typically contrastive explanations refer to ``why not?'' questions and
% consider counterfactuals, in our case the contrast is between the decisions
% made by two different policies.

\section{Background}
%%% RL and MDP %%%
For the purpose of this work, we assume a Markov Decision Process (MDP) setting.
Formally, an MDP is a tuple $\langle S,A,R,Tr \rangle$, where S is the set of
world states; {A} is the set of possible actions available to the agent; $R:S
\times A \rightarrow \mathbb{R}$ is a reward function mapping each state, and
$Tr(s,a,s') \rightarrow [0,1] \; s.t. \; s,s' \in S, \; a\in A$ is the
transition function.
% \begin{itemize} \item \textbf{S:} The finite set of world states. \item
%     \textbf{A:} The finite set of possible actions available to the agent.
%     \item \textbf{R:} A reward function $R:S \times A \rightarrow \mathbb{R}$,
%     mapping each state and action to a reward. \item \textbf{Tr:} A transition
%     probability function $Tr(s,a,s') \rightarrow [0,1] \; s.t. \; s,s' \in S,
%     \; a\in A$, defining the probability of reaching state $s'$ when
%     initiating action $a$ in state $s$. \end{itemize}
A solution to an MDP is a \emph{policy} denoted $\pi$. 
% An agent's policy is a
% mapping from states to actions such that for each state, a designated action is assigned.


%%% summaries %%%
\paragraph{Summaries}
%Ofra: we said this in the related work section

% Recent work introduced a new paradigm for conveying agent behavior ---
% \emph{``agent strategy summarization''}
% \cite{amir2018agent,amir2019summarizing}. In this paradigm, the strategy of an
% agent is described by demonstrating its actions in a carefully selected set of
% world states. 

% Such summaries can reduce the human effort required to review the agent's
% behavior, while still providing sufficient information about its capabilities.
% The key question in strategy summarization is then selecting the subset of
% situations, i.e. state-action pairs, to display. In other words which action
% sequences are most crucial in order to best portray the agent behaviour.

A summary, denoted $\mathbb{S}$, is a set of trajectories $T = \langle t_1,\dots t_n \rangle$.
% allowing for context surrounding the important state.  as opposed to singular
% states, in order to supply the user with richer context for the agent's
% behaviour in that state. 
Each trajectory $t$ being a sequence of $l$ consecutive states $t =
% \langle (s_i,a_i), \dots, (s_D,a_D), \dots, (s_{i+l},a_{i+l}) \rangle$
\langle s_i, \dots, s_D, \dots, s_{i+l} \rangle$
surrounding the disagreement state $s_D$ and extracted from the agent's
execution traces. 

We formally define a summary extraction process of an agent's policy given an
arbitrary importance function $Im$, mapping state-action pairs to numerical
scores.


\begin{definition}[Summary Extraction]
Given an agent's execution traces, a summary trajectory budget $k$, and an
importance function $Im$. \\
The agent's summary $\mathbb{S}$ is then the set of trajectories $T = \{
t_1,...,t_k \}$ that maximizes the importance function.
\begin{align}
    \mathbb{S} = \max_T \; Im(T)
\end{align}
\end{definition}
In this paper, our baseline is the HIGHLIGHTS algorithm, which computes
importance as a function of the $Q$-values in a given state. Specifically, we
implement the importance function from \citet{Tobias}, an extension to
HIGHLIGHTS, which suggests determining the importance of a state based on the
difference between the maximal and second $Q$-values.
% as opposed to the original HIGHLIGHTS importance function that was calculated
% between the maximal and the minimal values. 
Formally:
\begin{align}
   Im(s) = \max_a\; Q^\pi(a,s) - second\underset{a}highest\; Q^\pi(a,s)
\end{align}
The trajectory is then the sequence of states preceding and succeeding the
important state. 


==> sections/conclusion.tex <==
\section{Discussion and Future Work} \label{sec:conclusion} 
With the maturing of AI, circumstances which require people to choose between alternative market-available solutions, are likely to arise. The necessity of distinguishing between alternative agents becomes ever more clear. Moreover, distinguishing between policies is key for developers when analyzing different algorithms and  configurations. 

This paper presented a new approach for comparing RL agents by generating policy disagreement summaries. Experimental results show summaries help convey agent behaviour differences and improve users' ability to identify superior agents, when one exists. 


% These
% summaries emphasize the differences between agents, supporting people's a and helped people correctly identify the superior
% agent,  as shown in our experiment results. They also led to higher rates of confidence and
% explanation satisfaction rates.


% As the demand for intelligent agent solutions increases, so the supply is sure to follow. The
% necessity of distinguishing between agent behaviors becomes ever more clear. this paper proposes a
% new approach for comparing agents one against the other by generating summaries of the
% disagreements between them. These summaries magnify the differences between agents and help
% people, as shown in our experiment results, correctly identify the superior agent. 


% We now discuss several limitations of the developed \disalg~ algorithm and possible ways to address them, as well as additional directions for future work.

As for future work, we note the following possible directions: \textit{i)} expanding \disalg~ to enable comparison of more than two agents; \textit{ii)} testing additional state and trajectory importance methods; \textit{iii)} further enhancing the diversity between trajectories in the summary, and  \textit{iv)} formulating and defining disagreement ``types'' for generating further user-specific summaries.


%%% currently limited to two agents
% The current implementation of the algorithm can only compare two agents simultaneously, and these
% too have a required ordering of Leader and Disagreer. A natural first step would be obtaining a
% single summary that takes into account both configurations of Leader and Disagreer for each agent.
% Possible future directions to pursue would be making \disalg~ compatible for multiple agents by
% identifying common disagreements between all or generating some meta analysis between all pairs.

%%% mention other methods of importance
% We mention two methods for evaluating the importance of disagreement states (or trajectories), numerous others exist and are worth testing. 
% Some possible alternatives are:
% \textit{i)} evaluating the extent of the disagreement in a state through the second highest
% confidence value, in a fashion similar to the HIGHLIGHTS importance criterion; \textit{ii)} a
% summation over all states in a trajectory, \textit{iii)} observing the minimal and maximal values in
% a trajectory, and more. 

%%% diversity of disagreements
% Another direction we wish to pursue is enhancing the diversity between trajectories in the summary.
% We plan to identify key features of disagreement trajectories allowing us to formulate a distance
% function between states or trajectories. This will reduce the probability of similar trajectories
% appearing the summary. Doing so will remove redundant information, thus giving way to more
% informative trajectories.

%%% value based on agent estimation 
% The assessment of a state's value, i.e. importance, is currently a function of both agents'
% $Q$-values, which may differ significantly. In future work we will define more sophisticated methods
% for determining the ``ground-truth'' value of a state by exploring ways of assessing importance that
% do not rely solely on the judgment of the agent itself, for instance utilizing state features or
% aggregating previously compared agent valuations.


%%% disagreements in user specified areas or scenarios
% Finally, disagreements summaries provide users with the top-most important policy differences between agents. We plan on exploring methods for allowing users to obtain summaries of different disagreement types based on their preferences.

% however, in some situations, the desire may be for observing
% specific kinds of disagreements.
% We plan on allowing users to specify disagreement types they wish
% the summary to focus on, these will include location-based disagreements (e.g. in the river) and
% action-based disagreements (e.g. when the agent chooses the \emph{go-down} action). 
% This will
% provide users with specific information regarding the conflicts between the compared agents'
% strategies and will hopefully increase users' confidence in their choice of agent.  



==> sections/empirical_methodology.tex <==

\section{Empirical Methodology} 
\label{sec: emp}

%%%overview
To evaluate our method we conducted two user studies. The first was designed to
assess whether \disalg~ summaries help users identify the superior between two alternative agents, while the second user study examines whether such
summaries are useful for conveying agent behavior differences. In both studies we
use the HIGHLIGHTS algorithm as a baseline for comparison. We note here that
there is a significant difference between the output summaries of both methods
rooted in the fact that \disalg~ was designed for presenting two policies in a contrastive manner. This is achieved by portraying both agents simultaneously on the screen.
To our knowledge no other global explanation methods exist that directly compare
 policies and visualizes their differences to lay users.
% which we can compare to\footnote{\citet{Sequeira2020} propose additional
% criteria for generating alternative HIGHLIGHTS summaries, we chose to compare
% the vanilla version of the algorithm.}. 

%%%% empirical domain
\emph{Empirical Domains.} To evaluate our algorithm we generated summaries of
agents playing the game of Frogger \cite{Frogger_game} and controlling a vehicle
in a highway environment \cite{highway-env}. 

\textbf{Frogger} The objective of the game is to guide a frog from the bottom of
the screen to an empty lily-pad at the top of the screen. The agent controls the
frog and can initiate the following four movement actions: up, down, left or
right, causing the frog to hop in that direction. To reach the goal the agent
must lead the frog across a road with moving cars while avoiding being run over,
then, the agent must pass the river by jumping on passing logs. This domain
allows us to compare different agents in a setting with ground truth information
about agents' skill, i.e. game score.

\textbf{Highway} This domain consists of a busy highway with multiple lanes and
vehicles. The
agent controls a vehicle driving through traffic with the intent of avoiding
collisions. The agent can choose to move right or left (changing lanes),
increase or decrease velocity or stay idle, i.e. make no change. There is no
defined target the agent is required to reach, instead the road goes on
continuously. This property allows us to observe the agent's general behavior and preferences
instead of focusing on its progression towards reaching the goal.Screenshots from the \disalg~ output summaries displayed in Figure \ref{fig:
domains}. 


\begin{figure}[ht]
	\centering
    \frame{\includegraphics[width=0.7\columnwidth]{images/domains.png}}\\
	\caption{\centering{\textbf{Top}: Frogger; \textbf{Bottom}: Highway.\\ Red \& black rectangles represent different agents.}}
	\label{fig: domains}
	\vspace{-0.3cm}
\end{figure}

%%%% the agents
\emph{Frogger Agents.} We made use of the framework developed by
\citet{Sequeira2020} to test the \disalg~ algorithm on multiple configurable
agents of varying capabilities. Three different agents were trained using standard $Q$-learning \cite{watkins1992q}, based on the configurations provided by the framework. 
\begin{itemize}
	\item \textbf{Expert (E):} 2000 training episodes. Default rewards. Average
	game score: 110,000.
	\item \textbf{Mid-range (M):} 1000 training episodes. Default rewards.
	Average game score: 50,000.
	\item \textbf{LimitedVision (LV):} 2000 training episodes. Default rewards.
	Lower perception of incoming cars. Average game score: 55,000.
\end{itemize}
Agent performance was calculated by averaging the game score of ten
executions. Each agent's unique configuration contributes to its performance,
providing us a ground truth for the assessment tasks we present to the
experiment participants. The agents' skill hierarchy, based on their average
score, is as follows: $E>LV>M$. An important requirement for the
experiment was that all agents have a decent ability to play Frogger.
Prior to this study, we verified via an additional experiment that HIGHLIGHTS summaries are indeed useful for comparing Frogger agents that differ \emph{substantially} in their skills (see Appendix).
All HIGHLIGHTS and \disalg~ summaries were generated for fully trained agents, thus
reflecting their final policies. 


\emph{Highway Agents.}  Agents with varying behaviors were trained by altering their reward functions. All highway agents were trained for 2000 episodes using double DQN architecture
\cite{hasselt2010double} and rewarded for avoiding collisions.
\begin{itemize}
	\item \textbf{ClearLane (CL):} Rewarded for high velocity while maximizing the distance between
	itself and the nearest vehicle in front of it.
	\item \textbf{SocialDistance (SD):} Rewarded for maximizing the distance
	between itself and the closest $k$ vehicles.
	\item \textbf{FastRight(FR):} Rewarded for high velocity and driving in the
	rightmost (bottom) lane.
\end{itemize}
Henceforth,
we will refer to all domain agents by their abbreviations.

\emph{Summary Attributes}
% are listed in Table \ref{tb:parameters}. \ya{this moved to supplementary,
% mention that it's there or simply don't mention?}
All summaries were composed of five trajectories made up of sequential states, ten for Frogger and twenty for Highway. These contained the important state at the center of the
trajectory, with half the states preceding and the rest succeeding it.
Video-clips of the summaries were generated to present to the users and a
fade-in and fade-out effect was added to further call attention to the
transition between trajectories.
 For more details, sensitivity analysis and the complete surveys, see Appendix.
% \footnote{A summary of length 5
% was found useful in previous experiments with
% HIGHLIGHTS~\cite{amir18highlights}.}
% \footnote{Parameter sensitivity test appears in the Appendix.}
% \footnote{Parameter values used to generate
% summaries provided in the Appendix.}.


\paragraph{Experiment 1 - Identifying Superiority}
The objectives of the first experiment were twofold. Firstly, to support our
claims regarding the limitations of the HIGHLIGHTS algorithm for comparing
agents, and secondly, to compare the \disalg~ algorithm to HIGHLIGHTS and show
its added value. 

\emph{Hypotheses.} 
We hypothesized that summaries generated by the HIGHLIGHTS
algorithm are limited in their ability to help users distinguish between agents
and the \disalg~ algorithm is more suited for this task. More specifically,
we state the following hypotheses: \\
 \textbf{H1:} Participants shown summaries generated by HIGHLIGHTS for
 agents of decent skill will struggle to identify the better performing
 agent. \\
\textbf{H2:} Participants shown summaries generated by the \disalg~
algorithm will exhibit a higher success rate for identifying the better
performing agent, compared to ones shown HIGHLIGHTS summaries. 

%     \item \textbf{H3:} Explanation satisfaction of participants shown \disalg~
%     summaries will not be lower than that of participants shown HIGHLIGHTS
%     summaries (i.e. does not harm explanation satisfaction)\footnote{This hypothesis applies and was tested for both experiments}.
% 	\ya{maybe remove hypothesis about satisfaction?} \oa{definitely possible}



\emph{Experimental Conditions}
A between-subject experimental setup was designed with two experimental
conditions that varied in the summary generation method, \disalg~ or
HIGHLIGHTS~\cite{amir18highlights}. Participants were randomly assigned a
condition. 


\emph{Participants.} 74 participants were recruited through Amazon Mechanical
Turk (27 female, mean age $= 36.51$, STD $= 9.86$), each receiving $\$3$ for
their completion of the Task. To incentivize
participants to make an effort, they were provided a bonus of 10 cents for each
correct answer in the superiority identification task.
Participants who spent less than a threshold duration of time on experiment tasks, based on the length of the task summary video, were filtered out.

%%%% Procedure \emph{Procedure.} The experiments starts of by introducing
% participants to the game of Frogger, the concept of AI agents and to visual
% summaries as produced by HIGHLIGHTS. Each explanation was followed by a short
% quiz to ensure understanding before advancing to the task. Next, participants
% were faced with two stages of agent selection tasks, each followed by an
% explanation satisfaction questionnaire.

% \textbf{Part A: Comparing agents with a high degree of variation in skill} The
% first part of the experiment was designed to ensure that agents whose
% performance \emph{does} vary greatly are indeed distinguishable using the
% HIGHLIGHTS summaries. We further describe this task and its results in the
% supplementary material.

% \textbf{Part B: Comparing agents with a low degree of variation in skill:}  In
% this part of the experiment, 

\emph{Procedure.} Participants were first introduced to the game of Frogger and
the concept of AI agents. Each explanation was followed by a short quiz to
ensure understanding before advancing to the task. Next, participants were
randomly split into one of two conditions and were shown summary videos of pairs
of different agents generated using either \disalg~ or HIGHLIGHTS. 
% The pairs of agents shown to participants in this section were combinations of
%  $E$, $M$, $LV$ which all possess high game capabilities. (i.e. exhibit low
%  degree of variation in performance). 

Participants in both groups were first introduced to the summary method they
would be shown and were required to pass a quiz to ensure their understanding.
Participants were then asked to choose the better performing agent based on the
summary videos. They were able to pause, play and repeat the summary videos
without restrictions, allowing freedom to fully inspect the
summary before deciding which agent they believe is more skillful. Participants
were also asked to provide a textual explanation for their selection and to rate
their decision confidence on a 7-point Likert scale (0 - not at all confident to 6 - very confident). Overall, there were 3 pairs of
agent comparisons $\langle E,M\rangle \langle E,LV\rangle \langle LV,M \rangle
$. The ordering of the agent pairs was randomized to avoid learning effects, and
participants were also not told if the same agent appeared in multiple
comparisons, that is, they made each decision independently of other decisions.

% and 6 configurations when accounting for the order of the summaries shown.
% Each participant was shown one configuration of each agent pair combination,
% resulting in three overall comparisons.
Participants in the HIGHLIGHTS condition were shown a HIGHLIGHTS summary of each
agent (i.e. two separate videos, one for each agent.), while participants in the
\disalg~ group were supplied two configurations of the \disalg~ summaries. One
summary where the first agent is the Leader while the second is the Disagreer,
and the opposite summary, where the first agent is the Disagreer and the second
is the Leader. 
% That is, in both conditions participants were provided with two
% videos, each of the same number of trajectories: in the HIGHLIGHTS condition
% each video showed only one of the agents, while in the \disalg~ condition each
% video showed both agents (each with different Leader and Disagreer roles).
Upon
conclusion, participants answered a series of explanation
satisfaction questions adapted from \cite{hoffman2018metrics}. 

\emph{Evaluation Metrics and Analyses.} 
The main evaluation metric of interest was the success rate of identifying the superior Frogger agent with each summary method. We compare this metric across all the agent selection tasks given to participants. We also compare participants’ confidence in their decision.
% and show the differences between the confidence of the participants who
% succeeded in identifying the better agent using the \disalg~ algorithm
% compared to HIGHLIGHTS.
To compare the explanation satisfaction ratings given to the summaries, we
averaged the values of the different items normalizing in such a way that
higher values always mean that the summary is more helpful.
% while 1 it was not. We now report the results of the user study. We report the
% mean values and the $95\%$ confidence interval (CI) computed using the
% non-parametric Mann-Whitney $U$ test. In all plots the error bars correspond
% to the $95\%$ confidence intervals. The full experiment survey can be found in
% Appendix \ref{app: survey}
In all analyses we used the non-parametric Mann-Whitney $U$ test and computed
effect sizes using rank-biserial correlation. In all plots the error bars depict
the bootstrapped $95\%$ confidence intervals~\cite{efron1994introduction}. 
% T We use bootstrap non-parametric analysis~\cite{efron1994introduction} for
% the statistical tests. Plots show 95\% confidence intervals and we report the
% p-values for each comparison. %  but in all cases we state significant
% differences, the adjusted p-values were also smaller than 0.05. 


\begin{figure*}[t]
	\centering
	\includegraphics[width=0.85\linewidth]{images/successes_three.png}\\
	\caption{Participant Success Percentage per Summary Method. \textbf{DA:} DISAGREEMENTS; \textbf{HL:} HIGHLIGHTS.}
	\label{fig: DA HL compare}
\end{figure*}


\paragraph{Experiment 2 - Conveying Agent Differences}
This experiment's objective was to test the usefulness of \disalg~ summaries for conveying differences in general agent behavior in comparison to HIGHLIGHTS.

\emph{Hypotheses.} 
The \disalg~ algorithm is designed to portray instances of disagreement between
agents. We hypothesized that this would provide a clear and contrastive distinction between the alternative agents, thus emphasizing behavioral differences and providing a more appealing visual experience.
More specifically,we state the following hypotheses:\\ 
\textbf{H3:} Success rate of participants shown \disalg~  summaries will surpass that of participants shown HIGHLIGHTS summaries.  
\\
\textbf{H4:} participants will prefer summaries generated by the \disalg~ method.



\emph{Experimental Conditions}
A within subject setup was chosen in order to allow participants to provide a
direct comparison between the methods and state their preferences. As
participants experience both HIGHLIGHTS and \disalg~ summaries, to reduce cognitive overload, we chose to display only two agent comparisons for each
method. We chose the comparisons between the most distinctly dissimilar agents,
dropping $\langle SD,CL\rangle$ due to similarity of reward associated with
distance from neighboring vehicles. 

\emph{Participants.} 45 participants were recruited through Amazon Mechanical
Turk (13 female, mean age $= 37.51$, STD $= 10.35$), receiving similar pay and
bonus incentive as in the first experiment.
As in Exp\#1, participants were filtered out if their task completion time was below a threshold.

\emph{Procedure.} Participants followed a similar procedure as in the previous
experiment diverging solely in the domain introduction and the questions asked.
Instead of superiority between the agents, participants were queried about which
trait was more dominant in the compared agents. The ground truth was established
directly from the reward functions of the agents. Each comparison included two
such questions along with a mandatory confidence rating and textual explanation of the answers. In addition, participants were ultimately asked which method they preferred. Since this was a within-subject design, participants saw both methods, in a random order. All questions are provided in the Appendix.


\emph{Evaluation Metrics and Analyses.} 
The main evaluation metric of interest was the success rate of correctly assigning a more dominant trait to an agent. We compare this metric across the
different agent selection tasks and summary methods. Similarly to experiment 1, we compare participants’ confidence in their answers. For evaluating summary method satisfaction of participants we used the non-parametric Wilcoxon signed-rank test \cite{wilcoxon1947probability} for matched pairs.

==> sections/introduction.tex <==
\section{Introduction}
%%% motivation - general explanation of RL agents behavior
With the maturing of reinforcement learning (RL) methods, RL-based agents are
being trained to perform complex tasks in various domains, including robotics,
healthcare and transportation. Importantly, these agents do not operate in a
vaccum  -- people interact with agents in a wide range of settings. Effective
interaction between an agent and a user requires from the latter the ability to
anticipate and understand its behavior. For example, clinicians should
understand treatment regimes recommended by agents to determine their viability.

To facilitate improved user understanding of agents' behavior, a
range of explainable RL methods have been developed
\cite{XRL_survey,heuillet2021explainability}. These can be divided into two explanation categories: (1) ``local'' explanation approaches explaining why an agent chose
a particular action in a given state, e.g., saliency maps highlighting the
information an agent attends to~\cite{greydanus2017visualizing}, and (2)
``global'' explanation methods that describe the policy of an agent more
generally, such as strategy summaries that demonstrate the agents' behavior in a
selected set of states~\cite{amir2019summarizing}. While these approaches
have been shown to improve people's understanding of agent behavior,
they are typically not optimized for a particular user task.

%%% more specific motivation
In this work, we aim to enhance users' ability to distinguish between the
behavior of different agents. Such scenarios arise when people are required to
select an agent from a set of alternatives. E.g., a user might need to choose
from a variety of smart home assistants or self-driving cars available on the
market. Importantly, there often isn't a clear ``ground-truth'' for which agent
is superior, as agents may prioritize alternative outcomes and users may occupy
different preferences. For example, some users may prefer self-driving cars that
value safety very highly, while others might be willing to relax safety
considerations to a degree to allow for faster driving. The ability to
distinguish policies is also important for model developers, as different
configurations of reward functions and algorithm parameters can lead to
different behaviors in unexpected ways, especially in domains where the reward
function is not obvious, such as healthcare \cite{gottesman2019guidelines}. 

%%% existing policy summaries do not fully address the task of supporting agent
%comparison
One possible approach for helping users distinguish between policies of agents
is to use strategy summarization
methods~\cite{amir2018agent,amir2019summarizing}. 
% These methods demonstrate the behavior of agents in a selected set of
% world-states based on some criteria, such as the importance of a
% decision~\cite{amir18highlights,huang2018establishing}. Ofra: removed as we'll
% discuss this in related work or an ability to reconstruct the agents'
% policy~\cite{lage2019exploring,huang2017enabling}. 
Using these methods, a summary is generated for each agent, allowing the user to
compare their behavior. 
% While these approaches have been shown to be effective in portraying agent
% behavior, they are not optimized for
However, these approaches are not optimized for the task of agent comparison, as
each summary is generated \emph{independently}. For instance, the HIGHLIGHTS
algorithm~\cite{amir18highlights} selects states based on their importance as
determined by the differences in Q-values for alternative actions in a given
state. If two high-quality agents are compared, it is possible that they will
consider the same states as most important, and will choose the same (optimal)
action in those states, resulting in similar strategy summaries. In such a case,
even if the agents' policies differ in numerous regions of the state-space, it
will not be apparent from the summaries.

%%% the disagreements-based summary approach
This work presents the \disalg~ algorithm which is optimized for comparing
agent policies.
%%% we use Disagreements to...
Our algorithm compares agents by simulating them in parallel and noting
disagreements between them, i.e. situations where the agents' policies differ.
These disagreement states constitute behavioral differences between agents
and are used to generate visual summaries optimized towards showcasing the most
prominent conflicts, thus providing contrastive information. Our
approach assumes access to the agent’s strategy, described using a Markov
Decision Process (MDP) policy, and quantifies the importance of disagreements by
making use of agents’ Q-values.

%%% experimental results
To evaluate \disalg~, we conducted two human-subject experiment to test the following properties of the algorithm: Firstly, whether it improves users' ability to
identify a superior agent when one exists, i.e. given ground-truth performance measures. Secondly, do \disalg~ summaries outperform
HIGHLIGHTS summaries in conveying differences in behavior of agents to users.
% i.e.
% when superiority is not the name of the game.
Both
experiments make use of HIGHLIGHTS summaries as a baseline for comparison.
Results indicate a significant improvement in user performance for the agent
superiority identification task, while not falling short in the behaviour conveying task, as compared to HIGHLIGHTS.


% generated summaries comparing agents playing the game of Frogger
% \cite{Sequeira2020} % from the InterestingnessXRL framework
% \cite{Sequeira2020} and evaluated them in a human-subject experiment. We
% compare these summaries to ones produced by HIGHLIGHTS, which we use as a
% baseline. In the experiment, participants were shown summaries of different
% Frogger agents which varied in their performance. They were asked to select
% the better performing agent and answered explanations satisfaction questions.
% % They were also % asked to rate their satisfaction from the explanation
% method for the task of evaluating the agent’s % capabilities. Results show
% that \disalg~ led to improved user performance on the agent selection task,
% compared to HIGHLIGHTS. % ability of users to identify % the better performing
% agent compared to HIGHLIGHTSץ % , and increased explanation satisfaction
% ratings. % and increased the explanation satisfaction of % participants.

%%% summary of contributions
Our contributions are threefold: \textit{i)} We introduce and formalize the
problem of comparing agent policies;  \textit{ii)} we develop \disalg~, an
algorithm for generating visual contrastive summaries of agents' behavioral
conflicts, and \textit{iii)} we conduct human-subject experiments, demonstrating
that summaries generated by \disalg~ lead to improved user performance compared
to HIGHLIGHTS summaries.
% were preferred by participants and improved their ability to assess agent
% performance compared to the baseline summaries.\\


==> sections/results.tex <==
\section{Results}
We now describe the results of our comparison between the HIGHLIGHTS strategy summarization method and our novel \disalg~ approach. We report the main experimental results with respect to the hypotheses raised in the previous section. 

Figure \ref{fig: DA HL compare} shows the percentage of participants who were successful in answering the experiment tasks in each of the experiment conditions, for each agent pair combination.

\emph{(H1) Participants in the HIGHLIGHTS condition struggled to successfully identify the better
performing agent in the comparison task.} When all agents are of decent performance, we see the difficulty
of distinguishing between them manifest itself in a poor success rate.
Based on participants' textual explanations of the choice of agent, it seems they were concerned that agent $E$ was indecisive, e.g., ``[Agent $E$] seems very indecisive while ... [Agent $M$] seems to have a plan and is going with it.''. %,  ``... [Agent $E$] behaved more like a human.''
We hypothesize that these responses are a consequence of a single trajectory in agent $E$'s summary where the frog is seen leaping between logs in a seemingly indecisive manner. These results emphasize the limitations of independent comparisons.
% summaries and strengthen our claims regarding their limitations.
% \ya{changed, but didn't mention anything regarding a random guess, not sure it's necessary}

% A Bootstrap analysis shows that in such a case,
% selecting the better performing agent is \emph{not} significantly different from a random guess  ($p > 0.59$ for all agent pairs).

% with  $(p =
% 0.59)$ for $E$ vs. $LV$, $(p = 0.595)$ for $E$ vs. $M$ and $(p = 0.595)$ for $LV$ vs. $M$. 

\emph{(H2) Participants in the \disalg~ condition were more successful in the agent comparison
task}. Participants in the \disalg~ group 
% given the same agents to compare, 
showed vast improvement
in the ability to identify the better performing Frogger agent  (see Figure \ref{fig: DA HL compare}). The differences in success rate between conditions  were statistically significant and  
substantial for all agent comparisons ($E$ vs. $LV$: $p = 1.6^{-5}$; $E$ vs. $M$: $p = 1.7^{-5}$; $LV$ vs. $M$: $p = 0.018$). Textual explanations provide insights regarding how the
contrastive nature of the \disalg~ summaries helped participants decide which agent to choose, e.g. `` I preferred the path that ... [Agent $E$] was taking''; ``I felt that ... [Agent $E$] was making slightly stronger moves, and pushing ahead further''.



% Figure \ref{fig: DA HL compare} reports the comparison in the percentage of participants that were
% able to correctly identify the better performing agent between the HIGHLIGHTS and \disalg~ summary
% methods. Participants observing the HIGHLIGHTS summaries showed poor success results for comparing
% between agents $E$ and $LV$, strengthening our H1 hypothesis -- \emph{Participants shown
% HIGHLIGHTS summaries of low-varying performance agents were not always able to correctly select
% the most skilled agent.} Participant in the \disalg~ group, given the same agents to compare,
% showed vast improvement in the ability to identify the better agent, strengthening our H2
% hypothesis -- \emph{Participants shown Disagreement summaries of low-varying performance agents
% were able to correctly select the most skilled agent.} The analysis shows a statistically
% significant and substantial difference in performance when comparing \disalg~ to HIGHLIGHTS with
% $(p < 1.4^{-5})$ for $E$ vs. $LV$ and $(p < 0.15)$ for $E$ vs. $HV$.

% \ya{maybe add some of the user study comments} \oa{yes, it would be nice if you could show an
% example comment or two from DA participants that shows the direct comparison helped them}


% \begin{itemize}
% 	\item \textbf{`` I preferred the path that ... was taking''} 
% 	\item \textbf{`` I felt that ... was making slightly stronger moves, and pushing ahead
% 	further''} 
% 	\item \textbf{``Agent ... was clearly making better choices''}
% \end{itemize}
%%%other options:
% ``Agent two made better choices overall in both videos''
% ``Agent 2 made smarter moves as a whole''
% ``Agent one got himself dead in the second video, the choice is easy.''
% ``Agent..reached lily pad first... further ahead first..''



% The analysis shows statistically significant and substantial differences in performance when
% comparing user success percentage using \disalg~ compared to HIGHLIGHTS. \ref{fig: DA HL compare}


% \emph{(H1) Participants shown HIGHLIGHTS summaries of low-varying performance agents were not
% always able to correctly select the most skilled agent.}  Participants’ selection for this agent
% comparison task are shown in Figure \ref{fig: HL vote}. These results support H1. The graphs
% indicate an agreement between our study participants that agent $LV$ dominates agent $E$ which we
% know to be false. A likely cause of this outcome can simply be the different states each agent
% determines as important, which results in different summary trajectories shown. This strengthens
% our claims regarding the limitations of HIGHLIGHTS summaries for comparison tasks due to
% non-dependency between the agents. 


% \begin{figure}[ht] \centering \includegraphics[width=0.75\columnwidth]{images/HL_hard_vote.png}\\
%   \vspace{-0.7cm} \caption{Agent selection using HIGHLIGHTS with low-varying performance agents}
%   \label{fig: HL vote} \vspace{-0.2cm} \end{figure}


% \emph{(H2) Participants shown Disagreement summaries of low-varying performance agents were able
% to correctly select the most skilled agent.}  Participants’ selection for this agent comparison
% task are shown in Figure \ref{fig: DA HL compare}. These results support H2. Given the same agents
% to compare, we can see a vast improvement in the user's ability to identify the better agent. 




% \begin{figure}[ht] \centering \includegraphics[width=0.75\columnwidth]{images/DA_vote.png}\\
%   \vspace{-0.7cm} \caption{Agent selection using the \disalg~ algorithm on low-varying
%   performance} \label{fig: DA vote} \vspace{-0.2cm} \end{figure}

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.75\columnwidth]{images/success.png}\\
% 	% \vspace{-0.7cm}
% 	\caption{Agent selection success percentage}
% 	\label{fig: DA HL compare}
% % 	\vspace{-0.2cm}
% \end{figure}

\emph{(H3) A significant difference was found between success rates of participants in the conveying differences task}. Participants achieved a significantly higher success rate with the \disalg~ method in the $FR$ vs. $SD$ comparison ($p = 0.014$). Albeit, this was mostly a result of the low performance of HIGHLIGHTS in $Q1$ due to the $SD$ summary containing, coincidentally, only trajectories of the agent at the bottom lane. 
The inferior performance of \disalg~ in $Q1$ of $CL$ vs. $FR$  ($p = 0.187$) can be explained by summary trajectories where no vehicles were present in $CL$'s lane allowing it to drive faster than $FR$ and appear less considerate of keeping distance.
While not necessarily outperforming it, the \disalg~ is at least equivalently useful as HIGHLIGHTS, which was shown to be better than random~\cite{Tobias}.


% \emph{(H3) Explanation satisfaction of participants shown \disalg~ summaries was similar to that of
% participants shown HIGHLIGHTS summaries.} Participants’ distributions of scores for the explanation
% satisfaction were not statistically significant $(p_{exp\#1} = 0.17, p_{exp\#2} = 0.61)$.

\emph{(H4) No clear participant preference towards one summary method was observed.} Most participants answered that both methods were equally beneficial. However,
more participants found \disalg~ more \emph{helpful} and containing less irrelevant information than HIGHLIGHTS, while finding the latter more \emph{pleasing}.



% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.65\columnwidth]{images/sat.png}\\
% % 	\vspace{-0.7cm}
% 	\caption{User satisfaction of summary methods}
% 	\label{fig: sat}
% % 	\vspace{-0.2cm}
% \end{figure}

% \emph{Confidence of correct participants.}
% Figure \ref{fig: conf}  shows the confidence
% ratings of participants who made the correct choice.\footnote{We compare the confidence ratings of
% correct participants, as being confident in a wrong choice is not desirable.} Ratings were slightly higher in two of the comparisons for the \disalg~ condition, however, none of the differences were statistically significant. 
% The analysis shows $(p = 0.68)$ for $E$ vs. $LV$, $(p  = 0.08)$ for $E$ vs. $M$ and $(p = 0.15)$ for $LV$ vs. $M$. 

\emph{Confidence and satisfaction}
In both experiments no statistically significant differences were found between the confidence or satisfaction of participants in different conditions (See Appendix).



% \emph{Correct participants in the \disalg~ condition were more confident than correct participants
% in the HIGHLIGHTS condition.} In addition to the agent selection success rate metric, we measured
% participants’ confidence in their selections. Figure \ref{fig: conf}  shows the confidence ratings
% of participants who made the correct choice\footnote{We compare the confidence ratings of correct
% participants, as being confident in a wrong choice is not desirable.}, showing that correct
% participants in the \disalg~ condition were more confident than correct participants in the
% HIGHLIGHTS condition. This difference was statistically significant for two of the three agent pairs
% ($(p < 0.017)$ for $E$ vs. $LV$ and $(p < 0.005)$ for $E$ vs. $HV$). 
% and the analysis show an increase in confidence of participants exposed to the \disalg~ summaries,
% with $(p < 0.017)$ for $E$ vs. $LV$ and $(p < 0.005)$ for $E$ vs. $HV$.


% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.65\columnwidth]{images/conf.png}\\
% 	% \vspace{-0.5cm}
% 	\caption{Confidence of correct participants}
% 	\label{fig: conf}
% % 	\vspace{-0.2cm}
% \end{figure}

